Mean Field Approximation for solving QUBO problems

The Quadratic Unconstrained Binary Optimization (QUBO) problems are NP hard; thus, so far, there are no algorithms to solve them efficiently. There are exact methods like the Branch-and-Bound algorithm for smaller problems, and for larger ones, many good approximations like stochastic simulated annealing for discrete variables or the mean field annealing for continuous variables. This paper will show that the statistical physics approach and the quantum mechanical approach in the mean field annealing give the same result. We examined the Ising problem, which is an alternative formulation of the QUBO problem. Our methods consist of a set of simple gradient-based minimizations with continuous variables, thus easy to simulate. We benchmarked our methods with solving the Maximum Cut problem with the G-sets. In many graphs, we could achieve the best-known Cut Value.

==> MeanField v4/tables/G-set_benchmark.tex <==
%\begin{tabular}{l | l | l}
% set & our best result & best known\\
% \hline
% G1 & 11624 & 11624\\
% G2 & 11620 & 11620\\
% G3 & 11622 & 11622\\
% G4 & 11646 & 11646\\
% G5 & 11631 & 11631\\
% G6 & 2178 & 2187\\
% G7 & 2006 & 2006\\
% G8 & 2005 & 2005\\
% G9 & 2050 & 2054\\
% G10 & 1999 & 2000\\
% G11 & 560 & 564\\
% G22 & 13353 & 13359
%\end{tabular}

%\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l}
%set               & G1    & G2    & G3    & G4    & G5    & G6   & G7   & G8   & G9   & G10  & G11 &  G12 & G22   \\
%\hline
%our best result   & 11624 & 11620 & 11622 & 11646 & 11631 & 2178 & 2006 & 2005 & 2050 & 1999 & 560 &  554 & 13353 \\
%best known result & 11624 & 11620 & 11622 & 11646 & 11631 & 2178 & 2006 & 2005 & 2054 & 2000 & 564 &  556 & 13359
%\end{tabular}


\begin{tabular}{l|l|l|l|l|l|l}
set               & G1    & G2    & G3    & G4    & G5    & G6  \\
\hline
our best result   & 11624 & 11620 & 11622 & 11646 & 11631 & 2178 \\
best known result & 11624 & 11620 & 11622 & 11646 & 11631 & 2178 \\

\end{tabular}
\\[0.5cm]
\begin{tabular}{|l|l|l|l|l|l|l}
  G7  & G8 & G9 & G10 & G11 & G12 & G22\\
\hline
  2006 & 2005 & 2050 & 1999 & 560 &  554 & 13353\\
  2006 & 2005 & 2054 & 2000 & 564 &  556 & 13359
\end{tabular}

